Scheduling of Multicast and Unicast Services under Limited Feedback by using Rateless Codes

Many opportunistic scheduling techniques are impractical because they require accurate channel state information (CSI) at the transmitter. In this paper, we investigate the scheduling of unicast and multicast services in a downlink network with a very limited amount of feedback information. Specifically, unicast users send imperfect (or no) CSI and infrequent acknowledgements (ACKs) to a base station, and multicast users only report infrequent ACKs to avoid feedback implosion. We consider the use of physical-layer rateless codes, which not only combats channel uncertainty, but also reduces the overhead of ACK feedback. A joint scheduling and power allocation scheme is developed to realize multiuser diversity gain for unicast service and multicast gain for multicast service. We prove that our scheme achieves a near-optimal throughput region. Our simulation results show that our scheme significantly improves the network throughput over schemes employing fixed-rate codes or using only unicast communications.

==> sec1_introduction.tex <==
\ifreport
\newpage
\fi
\section{Introduction}\label{sec:intro}

Over the past decade wireless scheduling and control techniques
(e.g., opportunistic scheduling) have been developed to exploit
opportunistic gains under the assumption of accurate channel state
information (CSI) \cite{Eryilmaz05,Lin06}. However, obtaining this information is costly in terms of bandwidth, time, and power, and could result in
incurring large overhead. Therefore, a critical question is ``how to
optimally manage network resources in the absence of such
information?'' We aim to answer this question by using
\emph{rateless codes} to jointly control power allocation,
scheduling, and channel coding for downlink cellular systems with
imperfect (and possibly no) CSI at the transmitter.

Rateless codes are a class of flexible channel codes that do not
require specifying the code-rate before transmission. A rateless
encoder generates a (near) unlimited stream of coded packets from a
given size of message bits. The transmitter progressively sends
these packets to the receiver, until the receiver successfully
decodes the source message and sends an ACK to the transmitter.
A major merit of rateless codes is that they do not require knowledge
of the CSI at the transmitter. Rateless
codes automatically adapt their code-rate to the channel
quality during the transmission. Therefore, they are capable of attaining near-capacity
performance over unpredictable time-varying channels \cite{Draper09}.

The first practical realizations of low complexity rateless codes
are Luby Transform (LT) codes \cite{Luby2001} and Raptor codes \cite{Shokrollahi2006}
for erasure channels. %While erasure channels are a good model for
%application layer packet losses, they do not adequately characterize
%noisy wireless communications.
Practical rateless codes for time-varying noisy channels were constructed in
\cite{Etesami06,Zhong2009,Bonello2011}, which utilize
belief propagation (BP) decoding algorithms to realize a
near-capacity performance over a wide range of SNR. %statistical channel variations
 The complexity of the BP decoding algorithms increases
linearly with the block-size of rateless codes \cite{Etesami06}.
Rateless codes that simultaneously achieve the
capacity of Gaussian channels at multiple SNRs
were developed in \cite{Erez2012,Gudipati2011}. They use
a layered encoding and successive decoding approach to achieve linear decoding complexity. Recently,
a new type of rateless codes, called spinal codes, has been proposed
\cite{perry2012spinal}, which uses an approximate
maximum-likelihood (ML) decoding algorithm to achieve the Shannon
capacity over both binary symmetric channel (BSC) and Gaussian channel models. The complexity of this decoding
algorithm is polynomial in the size of message bits, but is still
exponential in the block-size~\cite{Balakrishnan2012}.\footnote{In
\cite{Balakrishnan2012}, the rate gap $\varepsilon$ from the
capacity is inversely proportional to the block-size $L$, and the
decoding complexity is exponential in $1/\varepsilon$.}

In rateless codes, if the block-sizes are allowed to be arbitrarily
large, the achievable rate will gradually approach the ergodic
capacity of the channel, at the expense of unbounded
decoding time~\cite{networkinformation10}. However, in practice, one
cannot use rateless codes with arbitrarily large block-sizes so as to
maintain manageable decoding time and complexity. Therefore, the
block-size of rateless codes can be viewed as a parameter to control
the throughput-complexity tradeoff.

We investigate the cross-layer design of downlink cellular
systems with imperfect (possibly no) CSI at the transmitter that
employ rateless codes to resolve channel uncertainty. Most of the prior work on cross-layer network control with
imperfect CSI was centered on fixed-rate codes,
e.g.,~\cite{Wenzhuo12,Aggarwal12}, which can achieve Shannon
capacity for a certain channel state. However, these schemes suffer
from channel outages or inefficient use of available channel rates,
since the CSI information is not perfectly known at the transmitter. In
contrast, rateless codes combat these issues by choosing their
decoding time on the fly, at the expense of additional decoding
complexity. Recently, scheduling and routing policies based on rateless
codes were proposed in \cite{Urgaonkar2011,Yang12} for time-invariant channel environments. Dynamic scheduling for incremental redundancy HARQ was
analyzed in \cite{Mehr2011} for fading channels, which still requires feeding back ACK and realized mutual information in each slot to update the transmitter queue.


%To keep the decoding complexity low, we explicitly incorporate
%time-average block-size constraints, and aim to maximize
%the system utility.
We explicitly incorporate time-average block-size constraints to keep the decoding complexity low and maximize the system utility.
% The block-size of a rateless code is determined by both the network control decisions and the unknown CSI over many time slots.
This utility maximization problem is challenging for two reasons: 1)
the block-size of a rateless code is affected by the network control
decisions of many time slots; and 2) the system is only partially observed because the accurate CSI is not available. Therefore, unlike
standard utility maximization
problems~\cite{Eryilmaz05,Lin06,Stolyar2005,Neelybook10}, this
problem is a constrained partial observed Markov decision problem
(CPOMDP), which is generally intractable due to the ``curse of
dimensionality.'' To that end, the following are the intellectual
contributions of our paper:
\vspace{-0.1cm}
\begin{itemize}
\item
We formulate and solve a new utility maximization problem for
downlink cellular systems, which utilizes rateless codes to
resolve channel uncertainty. We develop a low-complexity dynamic
network control scheme to attain a near-optimal solution to this
problem. By varying the power allocation and scheduling decisions
dynamically in each slot, our control scheme exploits the imperfect
CSI and realizes a multi-user diversity gain.
%Our scheme is shown to achieve better performance than schemes that use fixed-rate codes, by avoiding channel outages and utilizing the full channel rate more efficiently.
Our simulation results show that our scheme, by avoiding channel outages and utilizing the full channel rate more efficiently,
improves the network throughput by up to 68\%,
compared with the schemes based on fixed-rate codes. To the best of our knowledge,
{\em this is the first cross-layer network control scheme for rateless codes over time-varying noisy channels that does not require accurate CSI information}.
\item
One of our key technical contributions is in showing
that our network control scheme meets the time-average
block-size constraint of rateless codes. In doing so, we prove that
the second order moment of the block-size of rateless codes is
finite. This is accomplished by establishing a large-deviation
principle for the reception process of rateless codes, which is
difficult because the underlying Markov chain of our scheme has an
uncountable state space.
\item
Another technical contribution is in developing a generalized Lyapunov drift method to analyze the
performance of our network control scheme. Conventional Lyapunov
drift methods require minimizing the drift-plus-penalty of the
system in each slot. However, our network control scheme generates
an approximate drift-plus-penalty solution for only a portion of
time slots. Nevertheless, we show that our scheme deviates from the
time-average optimal utility of infinite block-size channel codes by
no more than $O(1/L_{av})$, where $L_{av}$ is the enforced value of the time-average
block-size of rateless codes. This opens the door of being able to trade complexity/delay for performance
gains. Moreover, the feedback overhead of our scheme is at most $1/L_{av}$ of that for fixed-rate codes when no CSI is available at the transmitter.% the absence of CSI.
\end{itemize}

%\subsection{Related Work}



==> sec5_simulation.tex <==
\section{Simulation Results}
We present simulation results of Algorithm NCA. In our theoretical
analysis, we assume that $\{\textbf{h}[t],\hat{\textbf{h}}[t]\}$ are
\emph{i.i.d.} across time. However, our proposed Algorithm NCA is
robust even for time-correlated wireless channels. To illustrate
this, we consider a first order autoregressive (AR) Rayleigh fading
process in our simulations. In particular, the channel states
$\{h_s[t],\hat{h}_s[t]\}$ are modeled by
\begin{eqnarray}
&&h_s[t+1] = \sqrt{0.1} h_s[t] + \sqrt{0.9} n_s[t],\\
&&\hat{h}_s[t] = \sqrt{\rho} h_s[t] + \sqrt{1-\rho} \hat{n}_s[t],
\end{eqnarray}
where $n_s[t]$ and $\hat{n}_s[t]$ are \emph{i.i.d.} circular-symmetric
zero-mean complex Gaussian processes, and $\rho$ represents the
accuracy of the imperfect CSI $\hat{h}_s[t]$. The mutual information
is expressed by $I(h_s,P)=\max\{\log_2(1+|h_s|^2P),I_{\max}\}$ \footnote{As we have mentioned, the additional upper bound $I_{\max}$ is due to the limited
dynamic range of practical RF receivers.}, and the utility
function is determined by $U_s(x_s)=\ln(1+x_s/K)$. The average
SNR is given by $E\{|h_s[t]|^2\}P_{av}=12$ dB.


Two reference strategies are considered for the purpose of performance
comparison: The first one uses infinite block-size channel codes
(or equivalently the genie-assisted policy in Section \ref{sec:performance}), which achieves the performance upper bound in problem \eqref{eq95}, but
is infeasible to implement in a practical system. The second one uses
fixed-rate channel codes, where the code-rate $R$ is selected to
maximize the goodput $R\Pr\{I(h_s,P)K\geq R|\hat{h}_s\}$. Network control
schemes are designed for these two reference strategies to maximize
their corresponding total network utility.
\begin{figure}
\centering
\includegraphics[width=3in]{varying_V_figurev2.eps}
\vspace{-0.1cm}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex
\caption{Simulation results of total network utility versus the algorithm parameter $V$ for $L_{av} =10$, $S=3$ and $\rho = 0.8$.} \label{fig1}
\vspace{-0.2cm}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=3in]{varying_Lav_figurev2.eps}
\vspace{-0.1cm}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex
\caption{Simulation results of total network utility versus the time-average block-size $L_{av}$ for $V =10000K$, $S=3$ and $\rho = 0.8$.} \label{fig2}
\vspace{-0.2cm}
\end{figure}
%The block-size of fixed-rate channel codes is fixed to be 1 to simplify the numerical optimization.


Figure \ref{fig1} compares the results of total network utility
versus the algorithm parameter $V$ for $L_{av} =10$, $S=3$ and $\rho
= 0.8$, where $K$ is the number of symbols in each packet, and ``CSIT'' stands for CSI at the transmitter. The performance of rateless codes first improves as $V$
increases, and then tends to a constant value. For sufficiently
large $V$, the total network utility of rateless codes is much
larger than that of fixed-rate codes and is quite close to that of
infinite block-size codes. Figure \ref{fig2} illustrates the
complexity/delay vs. utility tradeoff, as it plots the total network
utility versus the time-average block-size $L_{av}$ for $V =10000K$,
$S=3$ and $\rho = 0.8$. The performance of rateless codes improves
as $L_{av}$ increases. When $L_{av}\geq 2$, rateless codes can
realize a larger network utility than fixed-rate codes that are also
optimized for this system. Figure \ref{fig3} provides the results of
total network utility versus the CSI accuracy $\rho$ for $V
=10000K$, $L_{av} =10$ and $S=3$. The performance of all three
strategies improves as $\rho$ increases. When $\rho=0$, the
cumulative spectral efficiency of rateless codes and fixed-rate
codes are given by 3.246 bits/s/Hz and 1.93 bits/s/Hz, respectively,
which corresponds to a throughput improvement of 68\%.
\begin{figure}
\centering
\includegraphics[width=3in]{varying_rho_figurev2.eps}
\vspace{-0.1cm}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex
\caption{Simulation results of total network utility versus the CSI accuracy $\rho$ for $V =10000K$, $L_{av} =10$ and $S=3$.} \label{fig3}
\vspace{-0.2cm}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=3in]{varying_S_figurev2.eps}
\vspace{-0.1cm}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex
\caption{Simulation results of total network utility versus the number of receivers $S$ for $V =10000K$, $L_{av} =10$ and $\rho=0.8$.} \label{fig4}
\vspace{-0.2cm}
\end{figure}
When
$\rho=1$, the CSI ${\textbf{h}}[t]$ is perfectly known to the
transmitter, and we modify the encoding control scheme \eqref{eq87}
by choosing the message size as $M_s[n] =
I(h_s[t_{n,s}],P[t_{n,s}])K$ to eliminate the rate loss as in
problem \eqref{eq95}. By this, all three strategies achieve the same
performance. Finally, Fig. \ref{fig4} shows the network utility
results versus the receiver number $S$ for $V =10000K$, $L_{av} =10$
and $\rho=0.8$. The performance of all three strategies improves as
$S$ increases, which exhibits a multi-user diversity gain.


%\begin{eqnarray}
%M_s[n] = I(h_s[t_{n,s}],P[t_{n,s}])K,
%\end{eqnarray}
%which is equivalent to that of fixed-rate codes with no outage. \red{Yin, this is not clear? Why should the rate be the same as that of fixed rate codes?}


==> sec6.tex <==
\section{Proof of Theorem \ref{prop1}} \label{sec:analysis}
\subsection{Queueing System as a Markov Chain}
Let us define $T_s(t)\triangleq\sum_{t=t_{n,s}}^{t}1_{\{s(t)=s\}}$ as the number of slots that has been used to send the latest message of flow $s$. The evolutions of $T_s(t)$ is given by
\begin{eqnarray}
T_s(t+1)=
\left\{
\begin{array}{l l} 
T_s(t)+1_{\{s(t)=s\}},&~\textrm{if~} a(t)\neq s;\\
0,&~\textrm{otherwise}.
\end{array}\right.
\end{eqnarray}
We further define $\Upsilon_g(t)\triangleq\sum_{n=0}^{n_g(t)-1}L_g(n)$ as the accumulated block-length of the rateless codes of group $g$, which evolves as
\begin{eqnarray}
\Upsilon_g(t+1)=\Upsilon_g(t)+ (T_g(t)+1)1_{\{a(t)=g\}}.
\end{eqnarray}

Let $\mathcal {X}(t)\triangleq\{R_u(t),\Phi_s(t),R_{gj}(t),Q_s(t),Z(t),n_s(t),T_s(t),$ $\Upsilon_g(t)\}$ denote the system state. Since the state spaces of the CSI and transmission power are finite, one can show that the state space of $\mathcal {X}(t)$ is countable. In the NC-RC algorithm, the network control action $\{s(t),P(t)\}$ at slot $t$ is determined from $\mathcal {X}(t)$ and $\hat{\textbf{h}}(t)$. Then, the service update variable $a(t)$ is determined from $\mathcal {X}(t)$, $s(t)$, $ P(t)$, and the channel states $\{h_u(t),h_{gj}(t)\}$. Then, one can observe that the system state $\mathcal {X}(t+1)$ can be derived from $\mathcal {X}(t)$, $s(t)$, $ P(t)$, and $a(t)$. Therefore,
the process $\mathcal {X}=(\mathcal {X}(t) ,t\geq0)$ is a discrete-time countable Markov chain.



\subsection{Fluid Limits}
We now establish the fluid limit model of $\mathcal {X}$. %Since $R_s(t)$, $R_{gk}(t)$, and $I_g(t)$ are finite,
Let us define the norm of $\mathcal {X}(t)$ as $||\mathcal {X}(t)||\triangleq\sum_{s=1}^{U+G} Q_s(t)+Z(t)$, where $Q_s(t)$, $Z(t)\geq 0$ for all $t\geq0$.%
%$\sum_{s=1}^{U+G} |\Phi_s(t)|++\sum_{u=1}^U|R_u(t)|$ $+\sum_{g=U+1}^{U+G}\sum_{j=1}^{J(g)}|R_{gj}(t)|+\sum_{g=U+1}^{U+G}|I_g(t)|$.
~Let $\mathcal {X}^{(x)}$ denote a process $\mathcal {X}$ with an initial state satisfying
\begin{eqnarray}\label{eq:init_con}
||\mathcal {X}^{(x)}(0)||=x.
\end{eqnarray}

Let $A_s(t)\triangleq\sum_{\tau=0}^t\Phi_s(\tau)$ and $D_s(t)$ denote the accumulated arrival and departure bits at queue $Q_s$ up to slot $t$, respectively.~We adopt the convention that $A_s(0)=0$ and $D_s(0)=0$.
Let $\Psi_s(t)\triangleq M_{s}1_{\{a(t) =s \}}$ denote the service rate of $Q_s$ at slot $t$.~Since the queue can be empty when it is scheduled, we have $D_s(t)-D_s(t-1)\leq \Psi_s(t)$.
The queue length $Q_s$ can be described in an alternative form
\begin{eqnarray}\label{eq:queue_evo1}
Q_s(t)=Q_s(0)+A_s(t)-D_s(t).
\end{eqnarray}

Let $W(t)$ and $V(t)$ denote the accumulated arrival and departure power of the virtual queue $Z$, respectively.~Therefore, we attain $W(t)\triangleq\sum_{\tau=0}^tP(\tau)$ and $V(t)-V(t-1)\leq P_{av}$.~Then, the virtual queue $Z$ can be also written as
\begin{eqnarray}\label{eq:eq1}
Z(t)=Z(0)+W(t)-V(t).
\end{eqnarray}

Let $B_{mi}(t)$ denote the time fraction up to slot $t$ when the network control action is $\omega_m$ and the imperfect channel state is $\hat{\mathbf{h}}_i$, defined by
\begin{eqnarray}\label{eq:eq20}
B_{mi}(t)\triangleq\sum_{\tau=0}^t1_{\{\omega(\tau)=\omega_m,\hat{\textbf{h}}(\tau)=\hat{\textbf{h}}_i\}}.
\end{eqnarray}

Let us define another process $\mathcal {Y}=(R_u,R_{gj},Q_s,A_s,D_s,Z,$ $W,V,B_{mi},\Phi_s,\Psi_s)$, where the tuple denotes a list of processes.~Therefore, the sample path of $\mathcal {Y}^{(x)}$ uniquely define the sample path of $\mathcal {X}^{(x)}$.~ We extend the definition of $\mathcal {Y}$ to each continuous time $t\geq0$ as $\mathcal {Y}^{(x)}(t)=\mathcal {Y}^{(x)}(\lfloor t \rfloor)$.

Recall that a sequence of functions $f_n(\cdot)$ is said to converge to a function $f(\cdot)$ uniformly over compact (u.o.c) if for all $t\geq0$, $\lim_{n\rightarrow\infty}\sup_{0\leq t'\leq t}|f_n(t')-f(t')|=0$. We now consider a sequence of processes $\{\frac{1}{x_n}\mathcal {Y}^{(x_n)}(x_n\cdot)\}$ that is scaled both in time and space, and show the convergence properties of the sequences in the following lemma:
\begin{lemma} \label{lem1}
With probability one, for any sequence of the processes $\{\frac{1}{x_n}\mathcal {Y}^{(x_n)}(x_n\cdot)\}$, where $x_n$ is a sequence of positive integers with $x_n\rightarrow\infty$, there exists a subsequence $x_{n_k}$ with $x_{n_k}\rightarrow\infty$ as $k\rightarrow\infty$ such that the following u.o.c convergences hold:
\begin{eqnarray}
&&\frac{1}{x_{n_k}}Q_s^{(x_{n_k})}(x_{n_k}t)\rightarrow q_s(t),\label{eq:uoc1}\\
&&\frac{1}{x_{n_k}}A_s^{(x_{n_k})}(x_{n_k}t)\rightarrow a_s(t),\label{eq:uoc5}\\
&&\frac{1}{x_{n_k}}D_s^{(x_{n_k})}(x_{n_k}t)\rightarrow d_s(t),\label{eq:uoc6}\\
%&&\frac{1}{x_{n_k}}Q_g^{(x_{n_k})}(x_{n_k}t)\rightarrow q_g(t),\label{eq:uoc2}\\
%&&\frac{1}{x_{n_k}}\hat{Q}_g^{(x_{n_k})}(x_{n_k}t)\rightarrow \hat{q}_g(t),\label{eq:uoc3}\\
&&\frac{1}{x_{n_k}}Z^{(x_{n_k})}(x_{n_k}t)\rightarrow z(t),\label{eq:uoc4}\\
%&&\frac{1}{x_{n_k}}\hat{D}_g^{(x_{n_k})}(x_{n_k}t)\rightarrow \hat{d}_g(t),\label{eq:uoc7}\\
&&\frac{1}{x_{n_k}}W^{(x_{n_k})}(x_{n_k}t)\rightarrow w(t),\label{eq:uoc8}\\
&&\frac{1}{x_{n_k}}V^{(x_{n_k})}(x_{n_k}t)\rightarrow v(t),\label{eq:uoc9}\\
&&\frac{1}{x_{n_k}}B_{mi}^{(x_{n_k})}(x_{n_k}t)\rightarrow b_{mi}(t),\label{eq:uoc9}\\
&&\frac{1}{x_{n_k}}\int_0^t\Phi_s^{(x_{n_k})}(x_{n_k}\tau)d\tau\rightarrow\int_0^t\phi_s(\tau)d\tau,\label{eq:uoc10}\\
&&\frac{1}{x_{n_k}}\int_0^t \Psi_s^{(x_{n_k})}(x_{n_k}\tau) d\tau\rightarrow\int_0^t\psi_s(\tau)d\tau,\label{eq:uoc11}\\
%&&\frac{1}{x_{n_k}}\int_0^t \tilde{C}_s^{(x_{n_k})}(x_{n_k}\tau) d\tau\rightarrow\int_0^t\tilde{c}_s(\tau)d\tau,\label{eq:uoc12}
%&&\frac{1}{x_{n_k}}\int_0^t \Omega_g^{(x_{n_k})}(x_{n_k}\tau) d\tau\rightarrow\int_0^t\omega_g(\tau)d\tau,\label{eq:uoc12}\\
&&\frac{1}{x_{n_k}}\int_0^t P^{(x_{n_k})}(x_{n_k}\tau) d\tau\rightarrow\int_0^tp(\tau)d\tau,\label{eq:uoc13}
\end{eqnarray}
where the functions $q_s,a_s,d_s,z,w,v,b_{mi}$ are Lipschitz
continuous in $[0,\infty)$.
\end{lemma}
\ifreport
\begin{proof}
See Appendix \ref{App:lem1}.
\end{proof}
\else
The proof of Lemma \ref{lem1} is provided in \cite{report_Sun2014}.
\fi

Since the limiting functions $q_s,a_s,d_s,z,w,v,b_{mi}$ are Lipschitz
continuous in $[0,\infty)$, they are absolutely continuous.~Therefore, these limiting functions are differentiable at almost all time $t\in[0,\infty)$, which we call \emph{regular time}.

%\subsection{Fluid Model Equations}
\begin{lemma}\label{lem2}
Any fluid limit $\{q_s,a_s,d_s,z,w,v,b_{mi}\}$ satisfies the following equations:
\begin{eqnarray}
&&q_s(t)=q_s(0)+a_s(t)-d_s(t),\label{eq:fluid_eq2}\\
&&a_s(t)=\lambda_st,\label{eq:fluid_eq1}\\
%&&\phi_s(t)=\lambda_s,\label{eq:fluid_eq3}\\
&&d_s(t)\leq\int_0^t\psi_s(\tau)d\tau,\label{eq:fluid_eq4}\\
&&\frac{d}{dt}q_s(t)=\left\{\begin{array}{l l}
\lambda_s-\psi_s(t), &\textrm{if}~ q_s(t)>0;\\
(\lambda_s-\psi_s(t))^+,&\textrm{otherwise},\end{array}\right.\label{eq:fluid_eq5}\\
&&z(t)=z(0)+w(t)-v(t),\label{eq:fluid_eq9}\\
&&w(t)=\int_0^tp(\tau)d\tau,\label{eq:fluid_eq10}\\
&&v(t)\leq P_{av}t,\label{eq:fluid_eq11}\\
&&\frac{d}{dt}z(t)=\left\{\begin{array}{l l}
p(\tau)-P_{av}, &\textrm{if}~z(t)>0;\\
(p(\tau)-P_{av})^+,&\textrm{otherwise},\end{array}\right.\label{eq:fluid_eq12}\\
%&& \sum_{m=1}^F \sum_{i=1}^E b_{mi}(t)=t.\label{eq:fluid_eq13}
&& \sum_{m=1}^F  b_{mi}(t)=\pi_it.\label{eq:fluid_eq13}
%&&e_s(t)=\int_0^t\tilde{c}_s(\tau)d\tau,
%&&\sum_{s=1}^S |q_s(t)| + \sum_{g=S+1}^{U+G} |q_g(t)|+\sum_{g=S+1}^{U+G} |\hat{q}_g(t)|+|z(t)|\leq1.\label{eq:fluid_eq13}
\end{eqnarray}
\end{lemma}
\ifreport
\begin{proof}
See Appendix \ref{App:lem2}.
\end{proof}
\else
The proof of Lemma \ref{lem2} is provided in \cite{report_Sun2014}.
\fi

Let us define the functions
\begin{eqnarray}\label{eq:fluid_eq3}
&&c_{mi}(t)\triangleq\frac{1}{\pi_i}\frac{d}{dt}b_{mi}(t),
%\\
%&&c_s(t) \triangleq \sum_{m:s^m=s} \sum_{i=1}^E c_{mi}(t)\pi_i,
\end{eqnarray}
for all regular time $t\geq0$. Then, by \eqref{eq:fluid_eq13}, we attain
\begin{eqnarray}
\sum_{m=1}^F c_{mi}(t)=1,~\forall~i.
%,\\\pi_i
%\sum_{s\in\mathcal {S}} \sum_{i=1}^E c_{s}(t)=1.
\end{eqnarray}

\begin{lemma}\label{lem3}
The fluid limit functions satisfy the properties:
\begin{eqnarray}\label{eq:lem3-1}
&&\psi_u(t)\geq \sum_{m:s^m=u} \sum_{i=1}^E \mathbb{E}\{I(h_u,P^m)K|\hat{\mathbf{h}}_i\}c_{mi}(t)\pi_i \nonumber\\
&&~~~~~~~~~~~~~~~~~~~~~~~~~~\times  \frac{M_s}{M_s+I_{\max}K} ,\label{eq:lem3-1}\\
&&\psi_g(t)= \sum_{m:s^m=g} \sum_{i=1}^E \frac{M_g}{\overline{L}_g}c_{mi}(t)\pi_i,\label{eq:lem4-1}\\
&&p(t)= \sum_{m=1}^F \sum_{i=1}^E P^mc_{mi}(t)\pi_i,\label{eq:lem5-1}
\end{eqnarray}
for all $u\in\{1,\cdots,U\}$ and $g\in\{U+1,\cdots,U+G\}$.
\end{lemma}


\ifreport
\begin{proof}
See Appendix \ref{App:lem3}.
\end{proof}
\else
The proof of Lemma \ref{lem3} is provided in \cite{report_Sun2014}.
\fi

\subsection{Stability Analysis}


%\begin{lemma}\label{lem3}
%The fluid limit functions satisfy the additional property:
%\begin{eqnarray}\label{eq:lem3-1}
%&&\int_0^t\psi_u(\tau)d\tau\geq \sum_{m:s^m=u} \sum_{i=1}^E \mathbb{E}\{I(h_u,P^m)K|\hat{h}_u\}~~~ \nonumber\\
%&&~~~~~~~~~~~~~~~~~~~~~~~~~~\times b_{mi}(t) \frac{M_s}{M_s+I_{\max}},\\
%&&\int_0^t\psi_g(\tau)d\tau= \sum_{m:s^m=g} \sum_{i=1}^E \frac{M_g}{\overline{L}_g}b_{mi}(t),\label{eq:lem4-1}\\
%&&\int_0^tp(\tau)d\tau= \sum_{m=1}^F \sum_{i=1}^E P^mb_{mi}(t),\label{eq:lem5-1}
%\end{eqnarray}
%for all $u\in\{1,\cdots,U\}$ and $g\in\{U+1,\cdots,U+G\}$.
%\end{lemma}



%\begin{lemma}\label{lem4}
%The fluid limit functions satisfy the additional property:
%\begin{eqnarray}
%
%\end{eqnarray}
%for all .
%\end{lemma}
%
%\begin{proof}
%See Appendix \ref{App:lem4}.
%\end{proof}
%
%\begin{lemma}\label{lem4}
%The fluid limit functions satisfy the additional property:
%\begin{eqnarray}
%
%\end{eqnarray}
%\end{lemma}

Let us consider a quadratic Lyapunov function for the fluid limit system:
\begin{eqnarray}
L(t)=\frac{1}{2}\sum_{s=1}^{U+G}{q}_s(t)^2+z(t)^2.
\end{eqnarray}
Then, we can establish the following statement:
\begin{lemma}\label{lem5}
Consider a network under the RNC-RC algorithm for any arrival rate vector $\bm{\lambda}$ strictly inside $\Lambda$. For any $\delta_1\geq0$, there exists an $\delta_2>0$ such that the fluid limit functions satisfy the following property with probability 1: At any regular time $t$,
\begin{eqnarray}
L(t)\geq \delta_1~ \textrm{implies}~ \frac{d}{dt} L(t)\geq -\delta_2.
\end{eqnarray}
\end{lemma}
\ifreport
\begin{proof}
See Appendix \ref{App:lem5}.
\end{proof}
\else
The proof of Lemma \ref{lem5} is provided in \cite{report_Sun2014}.
\fi

Now we are ready to prove Theorem 1. We first need to show that
\begin{eqnarray}\label{eq:3}
\limsup_{x\rightarrow\infty}\frac{1}{x} ||\mathcal {X}^{(x)}(xT)||\leq 1-\epsilon
\end{eqnarray}
holds with probability 1.

There must exist a convergent subsequence of ${x}$, i.e., $x_n$, that satisfies
\begin{eqnarray}\label{eq:4}
\lim_{n\rightarrow\infty}\frac{1}{x_n} ||\mathcal {X}^{(x_n)}(x_nT)||=\limsup_{x\rightarrow\infty}\frac{1}{x} ||\mathcal {X}^{(x)}(xT)||.
\end{eqnarray}
Lemma \ref{lem5} implies that for any $\zeta\in(0,1)$, there exists a finite $T>0$ such that $\sum_{s=1}^{U+G} |q_s(T)|+|z(T)|\leq\zeta.$ In other words, for any sequence of processes $\frac{1}{x_n}\mathcal {X}^{(x_n)}(x_nT)$, there exists a subsequence $x_{n_k}$ such that
\begin{eqnarray}\label{eq:2}
\lim_{k\rightarrow\infty}\frac{1}{x_{n_k}} ||\mathcal {X}^{(x_{n_k})}(x_{n_k}T)||\leq \zeta\triangleq1-\epsilon.
\end{eqnarray}
Since the sequence $x_{n}$ is convergent, its subsequence $x_{n_k}$ must converge to the same limit, i.e.,
\begin{eqnarray}\label{eq:5}
\lim_{k\rightarrow\infty}\frac{1}{x_{n_k}} ||\mathcal {X}^{(x_{n_k})}(x_{n_k}T)|| = \lim_{n\rightarrow\infty}\frac{1}{x_n} ||\mathcal {X}^{(x_n)}(x_nT)||.
\end{eqnarray}
Hence, \eqref{eq:3} follows from \eqref{eq:4}, \eqref{eq:2}, and \eqref{eq:5}.

%holds, because there must exist a subsequence of ${x}$ that converges to the same limit as $\limsup_{x\rightarrow\infty}\frac{1}{x} ||\mathcal {X}^{(x)}(xT)||$.

According to \eqref{eq:queue_evo1} and \eqref{eq:eq1}, we have
$||\mathcal {X}^{(x)}(xT)||\leq x + \sum_{s=1}^{U+G}A_s(xT)+W(xT)$. Hence,
\begin{eqnarray}
\mathbb{E}\left\{\frac{1}{x}||\mathcal {X}^{(x)}(xT)||\right\}\leq 1 + \sum_{s=1}^{U+G}\lambda_s T + P_{\max} T\triangleq F(T)\leq \infty.\nonumber
\end{eqnarray}
Therefore, it follows from the Dominated Convergence Theorem that
\begin{eqnarray}
&&\!\!\!\!\!\!\!~~~\limsup_{k\rightarrow\infty}\mathbb{E}\left[\frac{1}{x}||\mathcal {X}^{(x)}(xT)||\right]\nonumber\\
&&\!\!\!\!\!\!\!= \mathbb{E}\left[\limsup_{k\rightarrow\infty}\frac{1}{x}||\mathcal {X}^{(x)}(xT)||\right]\leq 1-\epsilon,
\end{eqnarray}
and thus the condition of Lemma \ref{lem4} is satisfied. This completes the proof of
Theorem \ref{prop1}.


==> sec6_conclusion.tex <==
\section{Conclusion}
We have attempted to answer an important question of how to
appropriately manage network resources in the absence of (or with
imperfect) CSI. To that end, we developed a cross-layer solution for
downlink cellular systems with imperfect CSI at the transmitter,
which utilize rateless codes to resolve channel uncertainty. To
keep the decoding complexity low, we explicitly incorporated
time-average block-size constraints in our formulation, subject to
which we maximized the system utility. Our network control scheme
jointly controls transmission power, scheduling, and channel coding,
and exhibits an elegant utility-complexity tradeoff. Our simulation
results suggest that rateless codes can improve the network
throughput by up to 68\% in certain scenarios, compared with
solutions that maximize the utility using fixed-rate codes.

